Relational Linear Programs

We propose relational linear programming, a simple framework for combing linear programs (LPs) and logic programs. A relational linear program (RLP) is a declarative LP template defining the objective and the constraints through the logical concepts of objects, relations, and quantified variables. This allows one to express the LP objective and constraints relationally for a varying number of individuals and relations among them without enumerating them. Together with a logical knowledge base, effectively a logical program consisting of logical facts and rules, it induces a ground LP. This ground LP is solved using lifted linear programming. That is, symmetries within the ground LP are employed to reduce its dimensionality, if possible, and the reduced program is solved using any off-the-shelf LP solver. In contrast to mainstream LP template languages like AMPL, which features a mixture of declarative and imperative programming styles, RLP's relational nature allows a more intuitive representation of optimization problems over relational domains. We illustrate this empirically by experiments on approximate inference in Markov logic networks using LP relaxations, on solving Markov decision processes, and on collective inference using LP support vector machines.

==> fol.tex <==
%!TEX root = main.tex
\subsection{First-Order Logic}
\label{fol}
A first-order knowledge base (KB) is a set of sentences or formulas in first-order logic \cite{genesereth1987logical}. Formulas are constructed using four types of symbols: constants, variables, functions, and predicates. Constant symbols represent objects in the domain of interest (e.g., people: \textit{anna, bob, chris}, etc.). Variable symbols range over the objects in the domain. Function symbols (e.g., {\tt MotherOf}) represent mappings from tuples of objects to objects. Predicate symbols represent relations among objects in the domain (e.g., {\tt Friends}) or attributes of objects (e.g., {\tt Smokes}). An interpretation specifies which objects, functions and relations in the domain are represented by which symbols. Variables and constants may be typed, in which case variables range only over objects of the corresponding type, and constants can only represent objects of the corresponding type. For example, the variable ${X}$ might range over people (e.g., {\textit{anna, bob}}, etc.), and the constant ${C}$ might represent a city (e.g., \textit{seattle}).

A term is any expression representing an object in the domain. It can be a constant, a variable, or a function applied to a tuple of terms. For example, \textit{anna}, {\tt X}, and {\tt GreatestCommonDivisor(X, Y)} are terms. An atomic formula or atom is a predicate symbol applied to a tuple of terms (e.g., {\tt Friends(X, MotherOf(}\textit{anna}{\tt))}). Formulas are recursively constructed from atomic formulas using logical connectives and quantifiers. If ${F1}$ and ${F2}$ are formulas, the following are also formulas: ${\neg F1}$ (negation), which is true iff ${F1}$ is false; ${F1 \land F2}$ (conjunction), which is true iff both F1 and F2 are true; ${F1 \lor F2}$ (disjunction), which is true iff F1 or F2 is true; ${F1 \Rightarrow F2}$ (implication), which is true iff F1 is false or F2 is true; ${F1 \Leftrightarrow F2}$ (equivalence), which is true iff F1 and F2 have the same truth value; ${\forall X F1}$ (universal quantification), which is true iff F1 is true for every object {\tt X} in the domain; and ${\exists X F1}$ (existential quantification), which is true iff F1 is true for at least one object {\tt X} in the domain. Parentheses may be used to enforce precedence. A positive literal is an atomic formula; a negative literal is a negated atomic formula. The formulas in a KB are implicitly conjoined, and thus a KB can be viewed as a single large formula. A ground term is a term containing no variables. A ground atom or ground predicate is an atomic formula all of whose arguments are ground terms. A possible world or Herbrand interpretation assigns a truth value to each possible ground atom.

A formula is satisfiable iff there exists at least one world in which it is true. The basic inference problem in first-order logic is to determine whether a knowledge base KB entails a formula ${F}$ , i.e., if ${F}$ is true in all worlds where KB is true (denoted by KB ${\models F}$). This is often done by refutation: $\mathrm{KB}$ entails ${F}$ iff KB ${\cup \lnot F}$ is unsatisfiable. (Thus, if a KB contains a contradiction, all formulas trivially follow from it, which makes painstaking knowledge engineering a necessity.) 

Inference in first-order logic is only semidecidable. Because of this, knowledge bases are often constructed using a restricted subset of first-order logic with more desirable properties. The most widely-used restriction is to Horn clauses, which are clauses containing at most one positive literal. The Prolog programming language is based on Horn clause logic \cite{lloyd1987foundations}. Prolog programs can be learned from databases by searching for Horn clauses that (approximately) hold in the data; this is studied in the field of inductive logic programming (ILP) \cite{lavrac1994inductive}.

First-order logic is especially convenient for representing relational structures like the social graph on Figure \ref{fig:friends}. All one needs is a pairwise {\tt friend(X, Y)} predicate with a ground atom for every edge and a unary ${\tt smokes(X)}$ predicate with a grounding for every smoker. On top of that ground KB concepts like \textit{has friends who smoke} or even \textit{shortest path to a smoking friend} can be easily model with logic formulas.

==> relLinProg.tex <==
%!TEX root = main.tex
\section{From Linear Programming to Relational Linear Programming}

Linear programs (LPs) have found a wide application in the fields of operations research, where they are applied to problems like multicommodity flow and optimal resource allocation, and combinatorial optimization, where they provide the basis for many approximation algorithms for hard problems such as TSP.  They have also
found their way to machine learning and AI. Consinder e.g. support vector machine (SVMs), which are among the most popular models for classification. And,
there are LP formulations of SVMs such as Zhou {\it et al.}'s LP-SVMs~\cite{zhou2002linear}. Many other max-margin approaches use LPs for inference as well 
such as LP boosting~\cite{demiriz2002linear} or LP-based large margin structure prediction~\cite{wang2009large}. In probabilistic graphical models LP relaxations 
are used for efficient approximate MAP inference, see e.g.~\cite{wainwright2008graphical}. Finding the optimal policy for a Markov decision problem can be formulated and solved with LPs~\cite{syed2008apprenticeship}. Likewise, they have been used for inverse reinforcement learning~\cite{ng2000algorithms} where the goal
is to estimate a reward function from observed behaviour. In addition, recent work use approximate LPs for relational MDPs~\cite{sannerB09}, which scaled
to problems of previously prohibitive size by avoiding grounding. However, they are not based on relational LPs.  Clustering can also
be formulated via LPs, see e.g.~\cite{komodakis2008clustering}. Ataman applied LPs to learning optimal rankings for binary classification problems \cite{ataman2007learning}. In many cases, even if a learning problem itself is not posed as an LP, linear programming is used to solve some intermediate steps. 
For instance Sandler {\it et al.}~\cite{sandler2005use} phrases computing the pseudoinverse of a matrix computation and greedy column selection from this pseudoinverse as LPs. The resulting matrix is then used for dimensionality reduction and unsupervised text classification. So what are linear programs?

%\input{lp}

